HapticLever: Kinematic Force Feedback using a 3D Pantograph

HapticLever is a new kinematic approach for VR haptics which uses a 3D pantograph to stiffly render large-scale surfaces using small-scale proxies. The HapticLever approach does not consume power to render forces, but rather puts a mechanical constraint on the end effector using a small-scale proxy surface. The HapticLever approach provides stiff force feedback when the user interacts with a static virtual surface, but allows the user to move their arm freely when moving through free virtual space. We present the problem space, the related work, and the HapticLever design approach.

==> 2-related-work.tex <==
\section{Related Work}
Large-scale haptic utilizing encountered-type interactions and robotic manipulators, and haptic approaches which make use of passivity through mechanical constraints.

\subsection{Kinematics Approaches}
\subsubsection{Large-Scale/Encountered-Type/Proxy-Based}

To provide realistic haptic sensations for body-scale or room-scale experiences, researchers have explored \textit{encountered-type haptics}, which aims to reconfigure physical environments in order to provide haptic sensations.

Encountered-type haptics is a paradigm in which the haptic touchpoint moves to the position of the virtual object and waits for the user to contact it.

The user is free to engage with or disengage from the touchpoint, and the control system of the touchpoint is concerned with repesenting the virtual object, rather than reacting to the user.

For example, TurkDeck \cite{Cheng2015TurkDeck} and HapticTurk \cite{Cheng2014HapticTurk} provided body-scale haptics through human actuation, in which human volunteers manually move a player or reconfigure static props within a physical environment.

Recent research has explored the use of \textit{robotic environments} providing similar haptic experiences.

For example, in RoomShift \cite{suzuki2020roomshift}, ZoomWalls \cite{yixian2020zoomwalls}, and MoveVR \cite{wang2020movevr}, ground-based robots are used to reconfigure physical environments and props providing a large-scale haptic sensations such as a wall, table, or furniture for room-scale haptic experiences.

On the other hand, TilePoP \cite{Teng2019TilePop} and LiftTiles \cite{Suzuki2019LiftTiles} explore how inflatable structures can support physical reconfiguration. 

REACH+ \cite{gonzalez2020reach} and HapticBots \cite{Suzuki2021HapticBots} utilize tabletop-scale robots to provide haptic feedback bound to a horizontal surface. 

More recently, Haptic Go Round \cite{huang2020hapticgoround} and CoVR \cite{Bouzbib2020CoVR} also explored the large-scale haptics. 



One clear benefit of these approaches is the stability of the haptic experience---since these devices are fully-grounded, they enable large-scale interactions such as pushing on, leaning against, or sitting on haptic props. 

However, the limitations of the room-scale encountered-type haptics are the high space requirements and high complexity they require.

\subsubsection{Mechanical Constraints}

Using mechanical constraints for VR haptics is a common approach among hand-scale devices.

Mechanical constraints are brakes or locks which stiffly hold a mechanism in a constant configuration, allowing the mechanism to sustain and transfer force without activating any motors.

The general advantage of using mechanical constraints for VR haptics is that the interactions are firm and stable and require minimal power consumption.

Wireality \cite{wireality2020} uses a mechanical brake on a string to stop a user's hand. DextrES \cite{Hinchet2018DextrES} uses an electrostatic brake to restrict the movement of fingers in a glove form factor. Electrostatic brakes are flat pads which strongly cling to one another when a high voltage is applied between the pads. 

Similarly, HapLinkage \cite{Li2020HapLinkage} uses mechanical latching between the two handheld controllers to lock their positions relative to each other.

Similarly, Grabity \cite{choi2017grabity}, Wolverine \cite{choi2016wolverine}, and DextrEMS \cite{Nith2021DextrEMS} also use the similar mechanical locks to provide haptic sensations.


\subsection{Dynamics Approaches}

Alternatively, large-scale haptics have been also explored using robotic arm-based approaches. 

In this scenario, instead of reconfiguring entire props or the physical environment itself, a haptic device provides a discrete touchpoint for the user as a representation of part of a virtual object.

Dynamics approaches are concerned with feedback control loops which incorporate force as an input or output signal. Dynamics approaches are concerned with applying certain forces on the user.

VRRobot \cite{vonach2017vrrobot}, Mantis \cite{Barnaby2019Mantis}, and Calvo \cite{calvo} are examples.

However, the primary limitation of the current approach is the integration of actuation into the mechanical arm.

The existing works actuate each joint directly to apply a desired force on the contact point.

These systems shake and oscillate when the user interacts with them. This is primarily because they comprise serial links and therefore suffer from the cantilever effect, and because they use a feedback control system which interfaces with the unpredictable, unmodellable human user.

These systems do not allow the user to move freely, even when the applied force should be zero; the user must fight the actuators in order to move the arm. Admittance control is sluggish and impedance control is resistive.

SnakeCharmer \cite{araujo2016snake} uses a serial robotic arm to provide an encounterable touchpoint for the user. However, because of the serial linkage design, the system has the cantilever effect.


==> 4-implementation.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Assets/Implementation}
    \caption{A labelled image of our implementation.}
    \label{fig:Implementation}
\end{figure}

\section{\system{}: Implementation}

To demonstrate our concept, we develop \system{}, a fully-grounded body-scale haptic system which employs the constant-scale lever mechanism and a height-changing small-scale plane constraint.
The geometry of this implementation is the case of the generalized design where $\alpha=0.216$.
Figure \ref{fig:Implementation} shows the overall mechanical design of \system{}.
The system consists of two parts: \textbf{\textit{1) a constant-scale lever mechanism}} constructed from aluminum profile and 3d printed parts; and \textbf{\textit{2) a height-changing dynamic constraint}} which moves a small-scale platform in one degree of freedom using a self-locking lead screw.
This section describes mechanical design, system implementation, and technical details of \system{}.

\subsection{Mechanical Construction}
The mechanical construction of \system{} is stiff, strong, and designed to be comfortable to use. 

\subsubsection{Materials and Construction}
%What materials did you use? %What housing, base, or supplementary structure did you create? %What type of filament did you use? %What are the characteristics of this filament?
We use one-inch extruded aluminum profile for the links and printed PLA fixtures for the joint coupling parts.
We use 8mm ID, 22mm OD bearings and 8mm steel rods for shafts where appropriate.
All of the parts for the constant-scale lever mechanism are easily obtainable.
The \system{} implementation is designed to minimize flexibility, and therefore maximize the interaction realism.
The primary source of flexibility in the design is play in the bearings; the one-inch aluminum profile is both strong and stiff, and the printed PLA parts are sized with a tight tolerance and securely fastened to the profile.
%What did you try? %What advantages does what you chose achieve? %How is everything connected? 
Users can position and orient their wrist in five degrees of freedom when holding the rotatable handle on the interface node. Because of the bearings and the fact that no motors are attached to the lever mechanism, users feel no resistance when moving the interface node around. However, the user must support the weight of the linkage.

The height-changing dynamic constraint comprises two linear motion sets, aluminum profile for the platform, DC motors, and printed PLA fixtures to connect everything together. 
Each linear motion set contains two 8mm steel guide rails, one 8mm lead screw, four rod clamps, two bearing blocks, two linear bearing blocks, one lead screw nut, and one aluminum block to attach to the lead screw nut. 
We use DC motors (FIT0521 with integrated encoder) to drive the lead screws and modify the plane position.
%What actuation system did you choose?
The lead screw system is mechanically self-locking, meaning that a force applied along the axis of the lead screw will not cause the lead screw to turn and the platform to lower. 
Yet, the DC motor is able to turn the lead screw, even when such an axial force is applied.
We control the motors using an Arduino Uno Rev3 and an Adafruit motor shield v2.1. 
We implement a simple proportional feedback controller to control the speed of the motors. 
The maximum speed of linear actuation is 1.6cm/s moving upwards and 2.0cm/s moving downwards.
Because the motion at the constraint node is scaled up, the maximum speed of the rendered plane is 7.5cm/s moving upwards and 9.5cm/s moving downwards.
In order for the constraint node to perceive any object as a fixed constraint, the object must be firmly fastened to the base node.
Therefore, we affix both the base node of the lever mechanism and the height-changing dynamic constraint to a construction of wooden two-by-fours.

\subsubsection{Technical Details}
% The overall cost of mechanical linkage component is [xxx] USD. 
% The size of the components is [xxx] cm in width and height. 
The weight of the linkage is 1.68kg, the weight of the entire HapticLever system including the base is 9.89kg, and the weight on hand which the user feels is 0.91kg.
The rotatable handle at the interface node gives the system five degrees of freedom. 
%What are the dimensions of the envelope?
The workspace of the interface node is a portion of a spherical shell with inner radius 342mm, outer radius 722mm, and solid angle 2.33 steradians. This workspace is large enough to prototype body-scale haptic interactions.


% The arduino receives commands from the simulation via usb.
%How does it receive commands/communicate with the simulation?
%What is the power draw of these electronics?
%what is the chain of events of receiving a command? %How long does it take?

\subsection{Integration with VR}
%How did you track things in space?
We use an Oculus Quest and Unity for our VR integration. 
Unity uses the Oculus Quest hand tracking feature to track the position of the interface node.
Because the design paradigm is passive and encountered-type, no command signal is or must be sent from Unity to the device when an actual collision occurs in the simulation.

%What were other options?
%What did you end up going with? %How did the tracking influence your design?

%What HMD did you use for your VR integration? %What program did you use to build your Vr simulation?
% ... Talk about the basics of the code that you implemented? %What is the pipeline for sending a command to the device? %How is the data transferred? %What happens when there is a collision with a virtual object? %What is the chain of events that happens when a virtual collision occurs? %What is characteristic of the continued action of interaction? %What happens at the end of the interaction?



==> 5-applications.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Assets/DemoApplications}
    \caption{The variety of demonstrations.}
    \label{fig:DemoApplications}
\end{figure}  


\section{Applications}

We show the versatility of the constant-scale lever mechanism by demonstrating what could be rendered using a different shape display from the one in the current prototype. The demonstrations are shown in Figure \ref{fig:DemoApplications} and include a horizontal plane, vertical planes, texture, an irregular surface, and drawing on a canvas with a stabilized hand. We achieve these different renderings by setting up the constraint node to interact with custom proxy objects.

%Horizontal plane
The \system{} implementation presented in this paper can render infinite horizontal planes at any height.
The self-locking lead screws ensure that the motors can move the small-scale planes by turning the lead screws, but that the user cannot move the planes by pushing on them.
Because the small-scale plane is mechanically locked and because the device is stiff, users can interact with the rendered plane naturally and comfortably. 
Users can press lightly on the rendered surface, press heavily on the rendered surface, slide their hand along the rendered surface, or hit the surface with an impact---and in all cases the surface will respond like a real table. 

%Vertical plane
\system{} can render vertical planes by setting up a vertical surface in the workspace of the constraint node. 
These vertical surfaces can be actuated similarly to how the horizontal plane is actuated in the current prototype, using self-locking lead screws.
This ensures that the interactions with the vertical planes are stiff and realistic.
This demonstration also features multiple intersecting planes, giving users the feeling of walls meeting at a corner or the inside of a box.

%Texture
\system{} can render textures by placing a textured material in the workspace of the constraint node.
The rendered texture felt by the interface node is a scaled up version of the texture of the original material. 
Users can feel the friction of a surface in addition to its shape characteristics.
A \system{} implementation could use a pin array shape display to dynamically change the rendered texture. 
Alternatively, the implementation could use a shape display on the surface of the constraint node, rather than on the surface which the constraint node touches.

%Irregular surface
\system{} can render an arbitrarily shaped object or surface by placing the object or surface in the workspace of the constraint node.
In the current implementation, the size and shape of the irregular surface is limited by collisions with the links of the lever mechanism.


%Drawing/Writing
\system{} can stabilize a user's hands on a virtual canvas and allow them to perform fine motor tasks such as drawing.
As Arora et al. shows \cite{Arora2017EvaluationOfSketching}, users have difficulty sketching and drawing in 3D VR space without any tangible or haptic constraint.
\system{} can provide a large drawing canvas to constrain the user's motion in a 2D plane so that the user can sketch easily and naturally.
The current prototype allows the user to position and orient their wrist with five degrees of freedom when gripping the interface node.
When a user interacts with a rendered plane, they then have four degrees of freedom: two translational and two rotational.
This reduction in the degrees of translational freedom while retaining rotational freedom, combined with the ability to press against the rendered plane and feel freedom, enables users to draw precisely.
This application is useful for collaboration in mechanical design and architecture fields, where designers architects can use the canvas to sketch their ideas and communicate.


%Squishy surface!!!!!!!!!! - active FF - easy?????



%How is the force feedback applied?
% The force which is felt by the hand takes the path through the end effector, through the linkage, and to the base joint and the pseudoplane contact. In the first path, the force travels through the base joint, through the wooden base, through the table or cart, and to the floor. In the second path, the force travels through the pseudoplane contact, through the pseudoplane, through the mechanically self-locking lead screws, through the wooden base, through the table or cart, and to the the floor. Thus, the force feedback interaction is mechanically constrained and the path of the force never passes through the motor. 
% %What have previous systems done?
% Previous systems either did not let users slider their hand along the rendered surface or presented resistance or impedance when the user was not intended to be feeling force feedback.
% %Why is that insufficient?
% Such interactions are unpleasant and unrealistic.
% %Where did you draw inspiration from?
% We drew inspiration from the realization that interacting with a boundary surface was less of a question of force rendering and more of a question of reduction of a degree of freedom of motion.
% %What are the final sizes of the parts? What are the sizes/characteristics of the gears, etc.? 


==> 6-user-study.tex <==
\section{User Study}

We conducted a pilot user study with 9 participants to assess the comfort and realism of our approach.
We asked participants to compare the \system{} prototype implementation, standard vibrotactile VR controllers, bare hands, and the ground truth of interacting with a real table.

\subsection{Participants}

We recruited 9 participants (2 female) aged 20-37 to participate in the study. All of the participants had used virtual reality previously. Three of the participants had previously used a force-rendering device. 
%If I want to do a quantitative study, do an analysis to see how many people I need to recruit. 
The study lasted thirty minutes and participants were compensated with \$20.

\subsection{Methods}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Assets/UserStudyUnitySubs}
    \caption{The application designed for the user study.}
    \label{fig:UserStudyUnitySubs}
\end{figure}

% we evaluate using questionnaires 
% we also noted participant thoughts using think aloud while they were using the different devices to gather insights 
% Experimental Setup & Procedure
%What did you ask the participants to do?
We asked participants to complete a task to wiping dirt off a table, shown in Figure \ref{fig:UserStudyUnitySubs}. To complete the task, participants had to erase 100 equally spaced dirt tiles from the surface of a $0.6\text{m}$ by $0.3\text{m}$ table. In each condition, participants completed the task on a $0.93\text{m}$ high table and on a $1.25\text{m}$ high table.
%What did the participants have to wear?
Participants performed the task standing up for all cases, and were allowed to move their bodies in order to reach the entire table.
%What hardware did you use?
Participants wore an Oculus Quest HMD for the study because of its hand tracking capabilities.


\subsection{Test Cases}
%If I want I can change this to having multiple test cases for each modality (horizontal plane, vertical plane, vertical plane at an angle) - this would try to allow each modality to show its strength

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{Assets/HapticConditions}
    \caption{The haptic conditions for the study. From left to right: The ground truth (a real table), a controller with vibrotactile haptic feedback, bare hands, and the \system{} implementation.}
    \label{fig:HapticConditions}
\end{figure*}

%How many conditions did you use?
We used 4 haptic conditions, shown in Figure \ref{fig:HapticConditions}, and 2 cases of different table heights for each condition.
%What was the baseline?
The baseline haptic condition was the ground truth of interacting with real table-like surfaces. The ground truth tables were the same heights and size as the virtual table. In this condition, users wiped small pieces of paper off of the table and did not wear the HMD.
%What implementation details are there about each of the cases?
Participants interacted with the implementation of our design paradigm facing the device, shown in Figure \ref{fig:HapticConditions}. Participants held the interaction node with one hand. The attachment at the interaction node allowed the user to move and orient their hand with five degrees of freedom. A researcher controlled the motors to adjust the height of the small-scale proxy plane to allow \system{} to render planes at different heights. In the \system{} condition, the Oculus Quest used hand tracking to determine when the user was contacting the table. Participants used the Oculus Quest controllers for the vibrotactile controller condition. The controllers vibrates whenever the users contacted the virtual table and whenever the participant erased a tile of dirt. In the bare hand condition, the Oculus Quest used hand tracking to track the participants' hands. In this condition, the only feedback the participants received when interacting with the table was visual feedback.
In all conditions, the virtual hand was bounded by the virtual table, and would not go below the surface of the virtual table even if the participant's hand was below the table height.
%How did you control the study (eg for noise?)

\subsection{Process}
Before beginning the study, we briefed participants on each of the haptic conditions they would be asked to use, and we communicated the safety risks associated with each condition. We communicated to participants that we would be recording their task times. Participants entered their demographic data and completed the Edinburgh Handedness Inventory \cite{Oldfield1971Handedness} prior to beginning the tasks. Participants were assigned the devices in a pseudorandom order.

%In each condition/test case, what did the users do?
In each haptic condition, users performed the wiping task on a high table and on a low table. 
%What did the users interact with in the application?
Participants erased dirt tiles by contacting the dirt tiles with their hands. 
%Did you randomize or confound anything? %Were there objectives or time limits?
%Did you use a think aloud protocol?
% We encouraged participants to think aloud during and between trials and we recorded their thoughts. We placed a text note in the virtual application reminding users to volunteer how the condition felt, how it compared with previous conditions, and what they wished for the current condition.
%Did you give out a questionnaire? 
Following the study, we asked participants to complete a questionnaire.
%What were the questions?
The questionnaire, taken from \cite{wireality2020}, asked users to evaluate the haptic conditions using the metrics of comfort, and realism. The questionnaire consisted of three seven-point likert scales with the questions: ``How realistic was the feeling of the surface?''---from \textit{Extremely Unrealistic} to \textit{Extremely Realistic}, ``How comfortable was the interaction?''---from \textit{Very Uncomfortable} to \textit{Very Comfortable},  and ``How free was your movement?''---from \textit{Blocked} to \textit{Full Range of Motion}.

\subsection{Results}
%The purpose of this study is more to get the qualitative feedback and to present it to the readers said they have an understanding of what it's like to use the device without having to actually use it rather than for me to draw conclusions I want to give the readers the information to be able to draw their own conclusions I can summarize findings 

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Assets/StudyResults}
    \caption{The study results.}
    \label{fig:StudyResults}
\end{figure}

The median laterality quotient among participants, from -100 being left handed to +100 being right handed, was 84.1. All participants were right handed and all participants chose to use their right hand for all tasks.
%Do you have a figure showing your results?
The median likert scale responses from the questionnaire are displayed in Figure \ref{fig:StudyResults}. 
%What kind of statistical test did you do? %Was there statistical significance? %What did you find? (Applying statistical results to context)
The ground truth was perceived as the most realistic while the bare hand condition was perceived as the least realistic. 
The ground truth and controller conditions were perceived as most comfortable while bare hands and \system{} were perceived as the less comfortable.
The bare hands, controller, and ground truth conditions were all perceived as free, while \system{} was perceived as least free.

%...Were you disappointed with the results? (Be honest) ... %So disappointing but not unexpected %Use the 'it's just a research device' scapegoat

\subsection{User Feedback}
%What were users' overall feelings?
Overall, 
\textit{``I was more than just that---other things---oh, cool, I can feel the thing in VR. This---let me feel it and \textbf{do} something, which is, I would say something I haven't done before.'' (P7)}.
Eight participants noted that the device was difficult to use, either because it was too heavy or awkward to hold
\textit{``You are holding something up---something that is somewhat weighty---with two of your fingers. And there's also a giant steel beam pushing down on it so it is not super comfortable too.'' (P5)}
\textit{``When you had it at certain angles, the force was slightly different ... when it was more bent forward, it wanted to keep going forward. So it was slightly off balance in that way'' (P6)}. %maybe not
\textit{``And I found that for me the haptic device was too heavy, so I felt like it was taking a lot of effort to lift it and to move it.'' (P2)}.
\textit{``In this case, I feel the cube motion---angle---it is a little bit uncomfortable because the cube is just only front or back. Yeah, I want a more free motion, like a GorillaPod'' (P3)}.
Six participants desired that their hand was free to orient any way that they wished, or desired that they had more freedom of motion of their fingers
\textit{``It feels like my hand was stopped, with the device, but it doesn't feel like it's being stopped on my hand. It feels like my hand is just suspended and can't move down. ...Because ... It feels like I'm holding a cube that just kind of stopped in midair, rather than touching a table. The feeling of the surface is there, but it doesn't feel like I'm touching a table.'' (P5)}.
\textit{``The freedom of range of your fingers is a lot better for the real one. For the device I have to hold the thing and know where I'm at. But I guess if it let my finger float freely but sort of maybe held my wrist back, then that way I would feel like there is a table---well no I guess your fingers could just pull. I don't know. I feel like there's a way if it let my hand move but it didn't let my arm move. That way I could really feel like I'm really like cleaning the table. Right now it felt like I was holding a ball and just rubbing it across the table.'' (P7)}.
\textit{``I think for the device, definitely adding the haptics on the hand or fingertips that would make it more cool. It gives me more feedback, just like the controller ones.'' (P9)}.
Four participants offered suggestions about how to improve the scenario and the virtual reality implementation
\textit{``You don't wipe some dirt with your game controller, right? ... I think you can change the virtual things---even if you hold a controller you could see your hand.'' (P1)}.
Six participants expressed that they found the bare hand condition significantly the worst.
\textit{``I was really surprised how terrible the free hand one was'' (P6)}.
\textit{``The vibration can give me some kind of feedback compared to the hand one. Yeah, the hand one was definitely the worst.'' (P9)}.
%Topical ground truth table 
One participant proposed that swiping bits of paper off a table was a good comparison to the VR scenario.
\textit{``I think paper may be the most similar thing you can find in real life: they are weightless, and in VR, yes---they don't have weight'' (P1)}.
\textit{``I think the surface area compared to the hand might be smaller ... I don't know if it's fair to compare the times because I just did like two swipes and it was all gone.'' (P2)}.
\textit{``I like it---it's the real one, the ground truth. But I don't like it because it doesn't have any virtual elements, it's not portable, it doesn't have anything imaginary.'' (P9)}.
Two participants said they were worried they would break the \system{} device.
\textit{``Um, the device---I was kind of afraid to break it.'' (P9)}.
Participants showed disagreement about which condition was most suitable for the task, though they agreed that the bare hand was worst for the task.
%What were some quotes from participants? %What did some users say they liked? 

%\textit{``Obviously there is more friction since you are dragging something across a surface'' (P5)}
%What comparisons did users make to the other cases?

%What undesirable feedback did users give? Why is that okay?

%What did participants think it might be useful for %What unexpected things did participants think it might be useful for? 

%I think the drawing/sketching thing is so widespread because of how I'm asking users to hold the device.
%What were some area of improvement noted by participants. 

%what participant expectations were shattered? 


%Why perform a  study? 
% While technical specifications can be validated through technical means, the justification for selecting criteria for a haptic system must be validated  through qualitative user testing. 
% The user study also reveals and records user feedback about how the device feels.
%We need to perform a a qualitative study in order or the readers to get some sense of what the device brings. We need to convey the personal interactive part of this haptic device.
%Should the wire-based system be wizard of oz? Multi-string haptics are good for complex geometries. I am not playing to their strength. I need more time if I am to create a good study
%I am leaving out an active linkage-based device. I don't have one. 


==> 8-conclusion.tex <==
\section{Conclusion}

Existing large-scale force feedback devices are either uncomfortable because they move sluggishly and with resistance or provide unrealistic interactions which are not stiff. The small-scale constraint can be a shape display, a small-scale proxy, or even an active force. \system{}  behaves stiffly when encountering the small-scale constraint and moves without resistance when not encountering the small-scale constraint.
\system{} lays a groundwork for promising future large-scale haptic devices that provide stiff and natural interactions.

==> old.tex <==
Abstract

% % %prev 'Marcus' paper
% % What
% We present a passive mechanical wearable force feedback device capable of rendering a static plane for room-scale VR haptic experiences. 
% % Why
% While there are many wearable haptic approaches, body-scale haptic interaction, such as touching or pushing a wall still remains a challenge. 
% % How
% In this paper, we propose a wearable haptic device, that can move freely in mid-air with three degree-of-freedom, but stops the movement when the user touches a vertical surface.
% We achieve this with [dynamic nonholonomic] mechanical approach that enables the completely passive (i.e., does not require any actuation parts such as motors) but stable and stiff enough for full-body-scale haptic interactions.
% We also incorporate this haptic device with haptic retargeting to enable more variety of interactions.
% This paper describes mathematical models, haptic interaction techniques, fully functional prototypes, technical evaluation, and user evaluation.
% We demonstrate the possibility of our haptic approach with body-scale interaction, such as walking in a maze, drawing on a virtual canvas, common VR input, etc. 



% %681 Report
% We present Feedbackpack, a novel backpack-worn mechanical force feedback device for virtual reality (VR) which passively enables users to interact with virtual planes. In the prior art, there does not exist a sufficiently transparent and stiff device which can be used for heavy force feedback in room-scale VR. Heavy force feedback increases realism, immersion, and physical exertion in entertainment applications and will open new avenues for research and training in industry. We discuss the suitability of this class of device for future force feedback applications. We present our iterative design process and an interactive mathematical model of our mechanism. We validate the prototype through a quantitative analysis of the strength, range, and stiffness of the device.


% %Dictation
% We present \System{}, a novel design paradigm for haptics which takes advantage of the encountered type paradigm and maintains portability through being active, yet supports passive interactions. This novel design paradigm can be used for grounded haptics as well as worn haptics. This device design fills a gap in the haptics space. This device goes around the downfalls of previous haptic devices. This design is designed to achieve what other devices could not achieve. We present the design and implementation of this design as well as comparing it with other devices or design paradigms conceptually. We present a user study comparing this device to other devices. We demonstrate the encountered type nature, the passive nature, and the active compensating nature of the design. As well, we demonstrate that the active nature can be used as active force feedback. %probably not
% We demonstrate applications for a basic implementation of the design




 
 
Introduction 

%Prev 'Marcus' paper
% Immersive technology promises advances in online collaboration, training, teleoperation, and entertainment. However, technology enabling realistic physical interaction lags the display technology. Realistic interaction can be characterized by the transfer of skills between the real and virtual worlds. In a realistic simulation, the user will be able to predictably apply their skills from the real world into the simulation. Likewise, in a realistic simulation, a user will be able to learn skills which they can then directly transfer to the real world. The end objective of realistic immersive technology is to enable experiences which are impossible or prohibitive to achieve in real life. For online collaboration, this means being able to draw, type, write, speak, and nonverbally communicate with collaborators with whom it is impossible to meet in real life. For training, this means learning and applying physical skills in in scenarios which it is cost-prohibitive or prohibitively dangerous to set up in real life. For teleoperation, this means receiving all relevant signals from the remote robot and operating it with full dexterity. For entertainment, this means encouraging skill-based proficiency and enabling lifelike experience of fictional, dangerous, or impossible scenarios.

% Current immersive technology implementations, called Virtual Reality (VR), comprise a head mounted display and independent handheld controllers. The handheld controllers have various button inputs, vibration feedback, and often have a sensing method for hand pose estimation. Common VR interaction techniques include moving around the tracked area, point and select, gaze based selection (estimated using head pose), grabbing (including picking up and dropping), and proximity based selection. Other less common techniques include speech recognition, path based input, and ...
% Current VR techniques use a combination of visual and vibration feedback for most physical interactions. Collisions with virtual objects (either static or mobile objects, and either directly through the embodied avatar or indirectly through held tools) will typically elicit vibration feedback as well as an appropriate visual interaction. Likewise, accelerating a held object often elicits similar feedback, proportional to the mass of the object and the speed of the tracked pose driver. Some implementations are able to provide rich vibration feedback. However, even these juicy interactions lack the 
%Possible interactions with physical objects include picking up, placing, dropping, throwing, pushing, 


Introduction 


% Any attempt to add force feedback to an immersive computing setup must be of net benefit to the experience. Currently, VR users are able to move freely in their tracked area. Any device which are not portable or whose workspace limits the user's freedom of motion are limiting their own application space severely. Generic force feedback setups must either be portable or must be integrated with a locomotion device.  

% Haptic force feedback devices can be categorized by either their technological approach or their supported interactions. Technological approaches include fully grounded versus body grounded versus ungrounded, active versus passive, mechanical versus string based, fluid power versus electric motors, and haptic illusions versus accurate force. Supported interactions include simulation of gravitational force, inertia, rotational inertia, shape, static presence versus force fields, and cutaneous haptics, the latter including heat, texture, and softness. Some of these parameters are linked. For example, active systems can only render force fields while purely passive devices typically render static surfaces.

% Active devices, such as the Phantom Omni, continually consume energy while providing force feedback. Active devices are able to render constant force, vibration, texture, and force fields. Force fields are used in rendering compliant surfaces and springs. The force feedback which active devices are able to give is limited by the motor specifications. Purely passive devices are unable to render constant force, vibration, texture, and force fields. Passive devices are able to render completely stiff walls. They can accept a light or a heavy force without changing their position beyond the elasticity of the mechanism. The maximum force that a passive system can provide is determined by the breaking strength of the mechanism. Systems driven hydraulically may be considered passive devices.
%admittance vs impedance devices - Denis Laurendeau paper
%clearly  a hybrid approach is ideal
% A primary challenge in haptics is maximizing the fidelity and breadth of enabled enabled scenarios while minimizing the haptic effort. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% 681 Report
% While immersive computing technology (Virtual Reality; VR) has been advancing rapidly and increasing in popularity, its applications are limited by the slower-paced development of haptics devices. State-of-the-art haptics for VR enable users to feel the size, shape, texture, and temperature of graspable objects. However, they do not support force-based interactions with virtual objects based on an objects’ weight, inertia, and static presence. These are fundamental interactions for feeling walls, lifting, swinging, and throwing objects, interacting with menus and application windows, and stabilizing a user’s hand. Stabilizing a user’s hand, in particular, is crucial for fine motor tasks such as typing, drawing, writing, and fine positioning of items.
% Traditional force feedback devices are fully-grounded desktop systems with limited operational range [1], [2]. Recent works have investigated portable and wearable systems. Ungrounded systems generate forces on the user through propellers [3], flywheels [4], ultrasound [5], or mobile robots [6]. Such devices are typically loud and unable to generate large forces. Body-grounded systems absorb the reaction forces into the user’s wrist, arm, or torso. These include haptic gloves [7], hand-grounded pinching devices [8], and torso-grounded upper body force feedback devices [9], [10]. To fit in with the landscape of modern immersive technology, modern haptic devices should be portable, namely handheld, worn, or integrated with a locomotion device.
% Recent wearable or handheld haptic devices which can render weight, inertia, or static presence include Wireality [11], Transcailbur [12], and a body-grounded robotic manipulator [10]. Wireality uses shoulder-mounted brakes to restrict strings attached to the hand, enabling the hand to perceive the shape and presence of a virtual object. This device cannot render forces perpendicular to the strings, prohibiting it from rendering weight or inertia. As well, because the device is purely passive, it cannot adjust to the user moving around in the real environment. Transcalibur uses a weight-shifting mechanism to dynamically simulate inertia with high fidelity. However, it is unable to render weight or static presence. The body grounded robotic manipulator can exert forces on the user’s hand in all directions, but suffers from lack of transparency, difficulty rendering static objects, insufficient refresh rate, and user discomfort.
% \subsection{Contributions}
% Feedbackpack contributes:
% \begin{itemize}
%     \item A haptic device to fill a gap in the force feedback application space, namely portable, passive interaction with immobile virtual surfaces
%     \item The technical design and validation of Feedbackpack, to serve as a foundation for future haptic devices
% \end{itemize}
% This artifact contribution is a novel force feedback design paradigm which implements an encountered-type interaction using a portable wearable device. Feedbackpack passively provides force feedback, dynamically controls its passive state, changes geometric properties to simulate inertia, and has the form of a mechanical linkage so as to be able to provide forces in all directions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%dictation
% Immersive computing is a door into endless possibilities. However, people' ability to interact with the virtual worlds remains limited. Over the decades, computing has given people the opportunity to make mistakes. The risk free environment of computing, has allowed trial and error, and unleashed creativity like no other technology. Immersive computing allows for the advantages of computing to be translated into embodied scenarios. However the lack of physical interaction in those scenarios severely detracts from the creative potential of the users and the breadth of applications.
% Haptics are necessary. Immersive computing is good. There exist haptic devices. A lot of them are hand based. you have to do texture, shape, heat, weight. So net forces on the hand... Forces on other parts of the body with texture and heat transfer. You have to do net moments on the hand for location of centre of gravity. It's not like there was general things have not been achieved. But it is a technological problem. Technologically, the approaches have not been sufficient. The others use admittance control or they are string based and they have inherent limitations or they are wrist based and they have inherent limitations in terms of generating net forces and moments or they use ungrounded force feedback which is loud and power hungry and unable to generate large forces and also is not a passive interaction or encountered type interaction and it can't render stiff things. 
% In this work we present , a new design for force feedback devices. In this design, the location of the force feedback, for example at the hand, is instead applied at the pseudo end effector.
% Let's start over logical progression I want to ground the forces I want to provide net forces on hand I want to provide moments on the hand you know give or take I want to provide stiff interactions I want to provide encounter type interactions that you don't need a name and admittance based device. James means I don't want an impedance based device and encounter type means I don't want an admittance based device
% I do want to carry the forces and if I don't want an ungrounded device which obviously I don't want because how are you going to get stiff interactions with an ungrounded device right how are you gonna get passive knock on the table interactions with an ungrounded device it's not impossible you would need super high bandwidth you would need super high forces you would need super amazing models of the person and you know compensation if there's any sort of off centeredness or where the force is being applied how are you passively be able to interact with the surface applying to start with at least so not ungrounded means that I've got to have some sort of linkage to carry the force you know some sort of mechanical member and that could be about or a string or a link strings of course have well strings and belts have the limitation that you can't push on a string so I gravitate towards a linkage OK well what then you know there are plenty of devices they use mechanical members to carry the force end you know hands this is not new you know the paradigm is not new you can have hand based devices club based or controller based devices basically any encounter type device well no that's not true most encounter type devices I don't know if that strider 
% % OK consider Lucas is device it has brakes kathy's device is basically the same as that Kathy sis on the shoulder and then kisses on the hand with both of these the break has to engage when the user gets to the point 
% % So something like Wolverine I suppose I need to check that out I need to figure out if it gets the the break the stopper into position before the user gets to that position because then you got something that is carried through a mechanical member Ann is stopped of course it's 1 degree of freedom and mine is 3 but it's not necessarily novel 
% In this work we propose hey linkage based mechanical force feedback device which has a mechanical mirror the end effector such that forces which are applied to the pseudo and affecter are felt on the end effector itself . Likewise the constrained motion of the pseudo end effector results in constrained motion of the actual end effector. We can achieve encountered type in passive interactions. As well the design allows for active and dynamic movement of the constraints that are being applied to the pseudo plane. Please woman replied in such a way that the force feedback interaction remains passive , through mechanical self locking systems 
% the primary principle of this design it is the force multiplication system or the positional movements multiplication system or scaling force and position scaling mechanism this mechanism allows us to constrain the motion and apply forces within a small volume and have that effect the end effector which is able to move over a large volume a basic device based on the paradigm to prove its capabilities 
% this device that we have created requires only position sensing it does not require force sensing therefore I suppose technically it fits into the category of an impedance device only it is exceedingly stiff and operates in that sense as an encounter type device Dixie so there are no for sensors it does not operate as an admittance based device nor does it use positioning sensing to look at the flex of the materials to infer force and therefore use admittance control The output signals are limited to motor positions the motor positions simply change the location of the founding planes and also adjust the position of the mountain plains said so to compensate for the movement of the device or the user if it is implemented as wearable devices designed for this purpose this dynamic system could itself be used as admittance based active force feedback system 
% Let's just be clear this is dynamic not active so active is it pushes back against the user to simulate AE positive restoring force or does positive work on the user to simulate positive work done in the virtual environment but this is just a dynamic device and the dynamic part of it is only to maintain the static position a virtual objects 
% in this paper we detail the types of existing haptic devices we explain why there is a need for further research why this is the logical next step why this solves a lot of the issues that current prices pose we go over the details of the design paradigm as well as the implementation of the proof of the concept represent a user study which has some objectives that I'm honestly kind of unclear about we present the demonstrations we discuss our findings based on our implementation and we discussed the errant limitations this designer as well we look at future work next steps possible applications possible form factors panda like 



Related Work


% Previous wearable force displays were string-based or active. String based displays allow transparent movement and support variable-force interaction, but do not support exerting forces in all directions. Body-scale active (impedance) devices using motors are not transparent and respond to changing forces by requiring a change in displacement. These explorations led us to ideate a design which employs a passive mechanical mechanism. This design operates as an encountered type device while also allowing forces to be applied in any direction.

% %from 681 paper draft:
% Force feeback devices are class of haptic technology which apply a force on the user to represent specific virtual objects phenomena. Because of Newton's second law, force feedback devices face inherent limitations based on, and can therefore be classified by, where they apply the equal and opposite reaction force. This work implements a body grounded passive force feedback device.


% \subsection{Fully Grounded Devices}
% Fully grounded force feedback devices apply the equal and opposite reaction force directly onto the static environment. Such devices may be securely attached to a desk, ceiling, wall, or floor. There are no fundamental limitations to which kinds of interactions this device can support. If implemented appropriately, fully grounded devices can support the user's weight, allowing the user to lean against a virtual wall, hang from a virtual bar, or freely walk on virtual terrain. The Geomagic Touch \cite{GeomagicTouch} is a desktop pen force feedback display. The user grasps a pen attached to a robotic arm and may probe or slide the pen along virtual surfaces rendered by the device. The Geomagic Touch is the commercially dominant desktop force feedback device. However, it suffers from a limited range of motion and a low maximum force. Snake Charmer \cite{SnakeCharmer} is a desktop robotic arm which moves to to location of a virtual object as the user's hand approaches. When the robotic arm moves into position, it stiffens so that it will remain stationary, regardless of how the user probes the end effector. This approach is called using an encountered device. Snake Charmer has multiple materials on its end effector which it can present to the user to simulate different textures. Holotron \cite{Holotron} is an example of a prototypes of a fully grounded full body force feedback device. These fully grounded fully body exoskeleton force feedback devices can simulate walking and running in addition to upper body interactions. These prototypes suffer from the cantilever beam effect, and the extremities of the exoskeleton are shown to shake and deflect.

% \subsection{Ungrounded Devices}
% Ungrounded force feedback devices apply the equal and opposite reaction force onto the surrounding environment without being attached to the environment mechanically. HapticDrone \cite{HapticDrone} allows a drone, connected to the user's hand by a string, to pull on a user's hand and apply force feedback. Thor's Hammer \cite{ThorsHammer} uses an array of controller-mounted fans to apply force feedback to a user's hand in any direction. Flywheel-based devices \cite{Okamura} applies the equal and opposite reaction force to accelerate or decelerate controller-mounted flywheels. UltraHaptics \cite{SonicHaptics} emits ultrasonic waves which hit the user's hand to render virtual objects. MoveVR \cite{Roomba} uses a wheeled mobile robot to pull on a string and exert forces on a user's hand. These devices are loud and are unable to render immobile virtual objects such as desks, walls, or doors. Most of these devices are only able to provide small forces in a limited range of direction. However, most of these devices are portable, allowing them to be used in room-scale VR.

% \subsection{Body Grounded Devices}
% Body grounded devices apply the equal and opposite reaction force onto a different part of the user's body. 
% %pinching devices
% %wrist-grounded
% %torso-grounded
% %shoulder-mounted
% %the one eyal was talking about
% %the one Ryo always mentions

% \subsection{Passive and Encountered-type Haptics}
% %Haptic serpent
% %Wireality
% %Capstan crunch??? Other wrist-based/pinch device?
% %

% \subsection{Body-Worn Haptics}
% %Repeat the body-grounded section but focus on how things are grounded to the body (methods-wise)

% %For thesis add section on FEMS

% \subsection{...}
% Our system moves beyond this...
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %from 681 final paper
% \section{Related Work}
% Force feedback devices are class of haptic technology which apply a force on the user to represent specific virtual objects phenomena. Body grounded force feedback devices, when applying a force on the user, apply the equal and opposite reaction force to another part of the user's body. This allows body grounded devices to be wearable, and therefore portable.

% HaptX gloves \cite{haptx} provide multimodal haptic feedback to the whole hand, including finger force feedback for rendering the shape of virtual objects. However, because the glove is grounded at the wrist, the device cannot generate the sensation of weight, inertia, or of an immobile object. Wolverine \cite{wolverine} is a hand mounted pinching device which uses mechanical locks to render graspable objects. When the locks are engaged, the system passively provides force feedback without consuming any energy. Wolverine is likewise limited to rendering massless, free-floating graspable objects.

% HapticSerpent \cite{HapticSerpent} is a wearable robotic arm which can pull at the user's clothes or brush the user with a feather to simulate haptics. This work focuses on the virtual environment interacting with the user, rather than the user interacting with the environment. HapticSerpent is worn using two straps, around the belly and waist, respectively.

% Wireality \cite{wireality} and HapticGEAR \cite{HapticGEAR} are torso-worn string-based force feedback devices. Wireality is worn on the shoulder using a backpack straps and a chest strap under the arms. HapticGEAR is a solid frame tightened onto the user's back with backpack straps. These string-based devices can provide passive force feedback when the strings are locked in position, but cannot provide forces perpendicular to the strings.

% Mantis \cite{mantis} and a masters thesis from MIT \cite{calvo} are over-the-shoulder robotic arms with handheld end effectors. The user continually grasps the end effector of the robot and moves through the back-torque of the joint motors. When force feedback should be applied, the joint motors activate and provide active force feedback. Consequently, if the robotic arm is rendering a virtual wall and matching the user's force, but then the user increases their force, the user will feel the wall move before the feedback control increases the reaction force from the robotic arm. Both of these devices are worn with simple backpack straps.

% Snake Charmer \cite{SnakeCharmer} and HapticBots \cite{hapticBots} are encountered-type desktop force feedback systems. This means that the system will move a physical proxy to the location of a virtual object that the user is about to touch. When the user expects to make contact, the physical proxy is there to passively provide force feedback. Encountered-type devices have the advantage that when the user is not experiencing force feedback, they may move their hand completely freely, without resistance or impedance.

% Our system moves beyond these, and implements a body grounded over-the-shoulder mechanical arm which can provide encountered-type passive force feedback in any direction.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% in force feedback our objective is to be able to render the forces that allow people to interact with virtual objects and environments in a way which gives them more creative freedom more ability to use their natural interaction inclinations 
% It's not just about realism it's about enabling better interactions certainly we start from the place of looking for things that exist in the real world we want to apply forces we interact with objects largely with their hands retouch we feel we grasp we pick up we throw me put down how do we achieve these interactions we need shape rendering you need to feel the texture of objects we need the softness of objects and I mean softness in terms of blankets not in terms of springs we need the heat transfer objects well that's good we also need the large forces the weight the rotational inertia we need the static presence of things like walls and tables and chairs that have high mass handheld objects we need the coordination of objects with other parts of our bodies we need two handed manipulation that is internally consistent ideally we need force feedback on all parts of the body you know in an ideal setting so with that Anne hit ourselves with objects and know where they are and not expect them to pass through our avatars how do we achieve these forces specifically given the shortfalls of current devices how do we achieve these larger forces wait which is the ever present force that objects apply on us when we are supporting their weight due to the gravity of the earth there is inertia which is the felt resistive force apply it on us when we accelerate object next which is just negative acceleration there is rotational inertia location of centre of gravity location of centre of gravity is just like wait in the sense that is an ever present moment which is on the hand if we are fully supporting an object that is due to the gravity pulling down on the centre of gravity of the object which is not directly over the hand then there is rotational inertia which is when we accelerate in object it generates the moment on our hands location of the centre of gravity so four things but then we also have static presence which is kind of its own category because picking up a plate is different than pushing on the countertop the interaction is totally different when you're working with high inertia totally grounded objects so let's focus on those forces newtons third law every action equal and opposite reaction any force or moment which is applied to the body must be applied on some other physical body such that F equals MA is satisfied therefore just force which is applied to the user the desired force has to be grounded it can either be fully grounded grounded to the earth the floor the roof it could be body grounded azraa spaces wrist based devices are it could be ungrounded. Let's just take a look at these to begin grander devices are like robotic arms which are screwed to a table the force which the user feels is on the other side transferred through for example the mechanical arm the mechanical linkage the mechanical links themselves through the table to the floor Body grounded devices such as where reality such as wrist based devices such as handheld devices send the reaction force to another part of the user's body which is totally fire ungrounded devices have a range of getaways that they achieve that sort of thing there are mobile robots which mate ground the force to the ground but not in a static way rather in a dynamically with wheels they might push on the air using the fans of a drone or they might push on the air using fans within a controller they might use ultrasonic waves they could use flywheels and store the energy .
% There are active and passive devices
% I am kind of stuck right now 'cause I don't know how to delete all of this out there are so many categories right there are so many categories and if I say I'm dividing the field in half with active and passive and then I'm dividing the field in half with mechanical instrument based then hey one of the ways that I have to phrase it is I divide the first half and then I divide in half again well am I taking the entire set and dividing in half or my taking one of the halves that I cut and dividing that in half .
% I should probably create a diagram or I should take all of the devices label them according to all of the dimensions put them all in a well then cluster them so after them then put the boundaries around it then put that as a figure then talk about the trends .
% I don't even know what active and passive means honestly active. Active means that when the force feedback is being applied there is current which is passing through a motor 2 achieve that force passive means when the force feedback is applied no energy is consumed or rather in an active device energy must be consumed 2 apply force feedback in the amount of energy consumed is proportional to the force perhaps because wraps for the device to function there might be an underlying amount of energy that needs to be consumed to run the system but it's not actually used for the force feedback in a passive device there might be an underlying amount of energy that needs to be consumed always but there's not any and then there might be like a step increase of energy to apply for us to be back to power this solenoid or whatever but it's not proportional to the amount of force feedback that is being applied it's you know or maybe a constant amount or something like that I don't know or think about it this way the system could not be designed or modified such that no force is renewable energy is required to apply the force mechanic on string based let's just do the definitions chemical in string based as mentioned before the forest has to be carried from the point where it's applied to the person two where it is eventually grounded whether that be the air or the person or the ground therefore should be transferred through multiple different their systems through multiple linkages or perhaps mechanical parts as well as strings but using judgment you can identify worth whether something is a string based device or mechanically based device subway streambase device means that the force which is being transferred is being transferred through a flexible member like a string or a belt or a chain. A mechanically based device transfers the force through rigid links . Forced to back devices should have some sort of actuation otherwise they can‘t model dynamic things in the virtual world and it operates more as a workstation then a robotic device I could stick with something instead of trying to break the rules see I'm having trouble coming up with this definition and here's the reason why if I say that this is only for active devices then where does my device fit in well it's an active device and a passive device how can I be not an active device is a dynamic device but if it's a dynamic device not an active device but it is a passive device and it uses actuation then actuation can't only be for active devices because mine is not active it could be active don't get me wrong it's just that's not what it's designed for OK certainly it's pretty clear like you can use electric motors to drive your actuation system or you can use fluid power which itself I guess is driven by fluid power or sorry you can use fluid power which I guess is driven by electric motors at the end of the day probably like you've got a piston you gotta motor you got a lead screw perhaps I could trace maybe that's a better idea I could trace system back I could say OK you have forced and you have the ground but then think about why reality OK it's a passive device not an active device and the well actually OK this is kind of a good good thing I kind of like this 

% OK so I left off on the other slide kind of thinking about a flow chart of where the forest goes or what are the crucial elements that carry or provide the force so in my device you have the user's hand and there's a force it's like a forced interaction system and that travels back through the mechanical linkages and it kind of works upwards to the other device third sorry to the other pseudo plane joint it works upwards so at the top of the part let me think about this again I have a picture in my head I should probably draw it out .
% At the top is no top is not the source bottom has to be this source which means at the top is the output oh this is so weird because in an encounter type device you're acting on this system as soon as an acting on you so it's all backwards think about why reality there's the user's hand there is a force which goes through the user's hand right from the front side to the backside I guess we're just on the front side because it's pulling on it then it goes through the strings right the strings are an integral part so if you take the strings out then it wouldn't work obviously although anything in that list is integral probably unless there's a parallel thing which is redundant this string is connected to a spool so this pool is carrying the forest but there's a mechanical break right a ratchet and that is carrying the force carrying the force but it is the part which is either there or not there so for example when I pull on the screen and there's no force feedback applied there's still some horse that's being transferred through this spring sorry through this string not a huge horse but there is a force and that there's a force from the inertia of this pool as it online but it kind of is there just with the inertia so looking at it in the braked position when you have the ratchet's locked the force goes through the mechanical system what am I saying I'm just rambling cousin trying to multitask make lunch the force the force goes through the ratchet and that is being pushed on Brian splendide right so I guess here there‘s how do I represent this in a flow chart because the force is perpendicular right the force on the ratchet is perpendicular to the force from the solenoid there's no component of the force which is being transferred through the strings through the everything which is being carried by the solenoid it's a completely separate new force I suppose except for the fact that economic years are you know one thing or the other when is the stolen it pushes it into place it doesn't need to continue acting it becomes a completely passive device which the user can disengage from so the force kind of ends there When the force is actually being applied you know that's the core interaction yes you couldn't look at it is there any actuation involved yet you have to engage the brake but is there actually enforce being applied I don't know Lucas is looking at locomotion systems more power his device though active about that active device in its current look you look at his device OK can you pull on the screen there's a force on the finger I presume and there is a force on the string cool kind of it kind of all the way through this bull actually hi my name is spool itself is being stopped by a motor but the motor has to be turned on for it to work if the motor is turned off… We're talking about food power this is supposed to be revealing power and the semantic hill that I ran into is that power is itself driven by electric motors why would you have a fluid piston ever why it adds a little tiny bit of squishiness but otherwise presumably you've got a leadscrew oh because sometimes you don't sometimes you have a pump right right sometimes you have a pump I forgot about that so it is not clear Just by looking weather in fluid power devices powered by a pump or a lead screw an electric motor still on his self worth Well there's one but there is another and the yolks are starting to come apart so standi Why is it important what is the effect of using premier Li electric motors versus food power Is that electric motors have back to work I guess nobody uses fluid power because people always hope that they can have well an impedance based device but if you have good power then you basically have to have space device I'm just gonna forget about blue power unless I find something the power to you know a good degree is just something that I looked into it something I looked into because I thought you wanted stiff interactions and electric motors just are not good enough for those different directions and maybe that's still true by fluid power might be you know reasonable in some respects right now I'm using lead screws will see if there's sufficient or if they're not maybe I'll leave the power to the related work sorry not related work the opposite future work section 
% I didn't talk about forcefield before when I talked about static presence I suppose should make a note that yeah you got gravitational force gravitational inertia inertia and rotational inertia shape rendering sure texture heat transfer softness heat transfer texture yeah static presence forcefields sharpness perhaps but static presence forcefields static presence is its own thing separate from the inertia you could model a high inertia thing but implementation wise it's better to tackle separately rotational inertia sorry that's not where I am at all forcefields forcefields it didn't mention it but these are like active forces at the restoring forces like springs or if someone throws a bullet you that's not it at all force fields position derived force magnitude and directions also known as impedance control 
% OK in terms of technical technological approaches haptic illusions versus force feedback which is not really dichotomous it's just a question of do they take advantage of optical illusions or do they actually try and represent horses inclusions are probably doing a combination of both why would you ever not use haptic illusions so you got like size weight you got positional illusions haptic retargeting you got exaggerated shapes like exrings I don't know what else within the related work it's worth talking about proxy objects how they fit into the categorization proxy updates are perfect yeah it's called real lag and we're trying to create a versatile system they can do things which are not real also if we have it internally then we can you know safety advise it I don't know I think I'm done with this let's move on 


% %Broadly, what research has been done.
% %What are examples of the breadth of research
% %What will you focus on? 

% %How would you categorize your current work (The categories can overlap and be at different scales)

% %talk briefly about the category?
% %...Just list the things and say what they can do??

% %See __ for a review

% %...


% %How does your system move beyond this prior worK?




Concept 



%Why is it important that the device is portable?
% The objective of this paradigm is to create a design capable of rendering large, stiff planes. This is a body-scale interaction. Thus, implementations of the design are best served as fully grounded devices alongside a locomotion system or as torso-grounded wearable devices. Torso-grounded wearable implementations must be portable, in that they must be able to account and compensate for user translation and rotation.
%Why is being active a requirement for being portable?





%What did you wish for the design goals to be? %What requirements must the device have, based on how it is to be used/implemented? 
%What are you doing for the rest of this section?
% In this section we discuss the development of these design goals and present the technical validation of our design concept.


% Feedbackpack uses a scaling mechanism, shown in \autoref{fig:conceptualDesign}, to achieve passivity. The primary linkage extends from the body grounding point to the handheld end effector. The scaling mechanism ensures that the scaled linkage moves in a perfectly scaled motion relative to the primary linkage. As a consequence, if the motion of the pseudo end effector of the scaled linkage is bounded to follow a certain path, the primary end effector will follow a scaled path. Feedbackpack uses this principle to set up a bounding plane at the pseudo end effector, called the dynamic pseudo bounding plane. If this pseudo bounding plane is mechanically locked to the base of the linkage, then the user's hand and the primary end effector will perceive a passive, encountered-type interaction with the apparent bounding plane.

% In the current iteration of the prototype, the pseudo bounding plane is statically mechanically  locked to the base of the linkage. However, Feedbackpack requires that this pseudo bounding plane be dynamic and actuatable. This is is important for both versatility and portability. An actuatable bounding plane will be able to render surfaces of varying distances and orientations. As well, an actuatable bounding plane will support portability by being able to compensate for the user's movement in the real world, ensuring that the real position of rendered virtual objects continually matches their virtual position. We plan to use self-locking lead screws to ensure that the pseudo bounding plane is both dynamic and continually mechanically locked to the linkage base.

% create a stiff system , AKA not an impedance system
% Create a transparent system, AKA not an admittance system 
% Create a system which can provide body scale forces while keeping the actuation profile volume envelope small 
% Minimize weight on hand 
% Allow large maximum forces. Note the variability in forces so being able to provide a light force or a heavy force in a passive way like as you do with a table or a static desk is envelope within the stiff system parameter because stiffness means that with the high change in force you do not see a high change in position 
% Design with the possibility of creating an active device in mind 
% Ensure portability by ensuring that the device can dynamically compensate for user motion and position. Specifically, see this has to do with the implementation now I have to have a separate set of design goals for the design paradigm and the implementation because you can have a better implementation like I think separating these is key crucial and I'm surprised that other papers don't do this as much. From a conceptual perspective yeah it has to be able to move and dynamically adjust so that it can maintain its position and conceptually the design itself can't have that inherent limitation of being unable to do that conceptual level . But the implementation you know has to prove that it's kind of possible in a reasonable manner but it doesn't have to be perfect and I get it saying I have an idea I can't prove it but I have an idea well that's useless But I can prove it analytically and I think that that's key here because then I can satisfy the wider range of what is possible at the far end of the spectrum and I can also toca Boo for the people who just want to see something working something that works kind of you know and it works OK fine 


% \begin{table}[tb]
%     \centering
%     \begin{tabular}{ccccc}
%          \toprule
%          Specification & Relation & Value & Units & Notes  \\
%          \midrule
%          Passive* & == & True & \\
%          Range of Motion & > & 70 & \% human range of motion & \\
%          Tolerable Force* & > & 700 & N & at handheld end effector \\
%          Stiffness* & > & 87.5 & N/mm & effective, measured at end effector \\
%          Viscous Damping* & < & 80 & kg/s & effective, measured at end effector \\
%          Natural Frequency & > & 200 & Hz & effective, measured at end effector \\
%          Weight on Hand & < & 375 & g & \\
%          Peak Power & < & 10.0 & W & \\
%          Position Control Overshoot & < & 2.5 & \% & \\
%          Position Control Settling Time & < & 0.1 & s & for perturbations up to 2mm \\
%          \bottomrule
%     \end{tabular}
%     \caption{The design specifications for Feedbackpack. Key specifications are marked with an asterisk (*).}
%     \label{tab:designSpecifications}
% \end{table}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.3]{Assets/passivityDemo}
%     \caption{A photo of the current Feedbackpack prototype.}
%     \label{fig:currentPrototype}
% \end{figure}


% are characterized by high stiffness. High stiffness means that is associated with low compliance. \ryo{need the explanation what the low compliance means.} If a haptic device must move through a force field to render something with high stiffness, then there is inherent compliance.


%Why is it important that the device is passive?
% The key advantage of the encountered-type haptics is to allow \textit{transparent movement} when it is not providing force feedback---the user can freely move without any constraints while not encountering the object.
% Therefore, encountered-type interactions allow the user to explore the rendered surface or object freely.
% While the most of wearable devices including our system, except for a few [HapticPivot] is difficult to achieve completely encountered-type interaction, it is possible to achieve the similar experience by leveraging the fully transparent movement during the interaction.

% The device's passive mechanical design allows it to fulfil the criteria of acting as an admittance device when providing force feedback and 
% The first key specification is that the device must be passive. This interaction paradigm allows the user to press with a large or a small force without displacing the render position. 
 
% %Why is it important that the device is encountered-type?
% % Thus, the device has the advantages of an encountered-type device while remaining wearable.
% % This design operates as an encountered type device while also allowing forces to be applied in any direction.

% %Why is it important that it is BOTH encountered-type AND passive? (SnakeCharmer/VRRobot are encountered type but not passive. Wireality is passive but not encountered-type
% The other big driver towards this design was the observation that interaction with surfaces is better modelled as loss of degrees of freedom rather than as a set of applied forces. That is, interaction with a surface does not care what forces you apply. It just cares where your hand can and cannot go.
% \ryo{I don't fully understand this paragraph.}


% Therefore, encountered-type interactions allow the user to explore the rendered surface or object freely.
% While the most of wearable devices including our system, except for a few [HapticPivot] is difficult to achieve completely encountered-type interaction, it is possible to achieve the similar experience by leveraging the fully transparent movement during the interaction.


%How do you know that it is encountered-type?
% The system fits the encountered-type abstraction because the plane or objects for the pseudoplane to interact with are put in the position to be interacted with and left there. 

%How do you know that there is not an excessive amount of weight or resistance during free movement?


% If a user is interacting with a rendered wall placed in front of them, and then steps forwards, the wearable device must now render the wall closer to the user. If the user is applying a force on the wall when they step forward, the the haptic device must to work on the user. Therefore, the subsystem of the design which places the plane to be encountered must also be able to adjust the location of that plane while doing work on the user.
% Therefore, the paradigm comprises a subsystem to place a plane to be encountered and a subsystem to transfer the encountering of that plane to be felt by the user's hand. The subsystem which places the plane must be able to do work on the user, yet must simultaneously be stiff and mechanically self-locking.
% The subsystem which transfers the force must be rigid and stiff.




Implementation


%What detail did you include to make it all work smoothly?
%How does the user's hand interact with the device? 
%What different things did you try? 
%What would have to happen for more complex interactions?
%What is complex about what you chose?
%Did you iterate through pilot studies?
%What is bad about the existing solutions


%Did you run tests to characterize the system?
%What are you talking about here? (test procedures/results/discussion)

%Is weight important?
%Why is weight important?
%What is the weight of your system?
%How is this mass carried?
%What is a good weight comparison?

%How much force can the thing withstand? 
%How much ... 












































































% % 681 Report
% \section{Evaluation}
% This evaluation serves as validation of the design specifications and implementation. The current prototype was intended to serve the purpose of verifying the conceptual design's passivity, range of motion, and theoretical force tolerance.

% \subsection{Passivity}
% The verification method for passivity is demonstration using the Feedbackpack prototype. \autoref{fig:currentPrototype} shows a user pulling on the primary end effector and feeling the force of a perceived bounding plane. Because this prototype does have any electrical components, it is clear that this force feedback does not consume any energy. Furthermore, when the user changes their applied force, the displacement changes negligibly and the power consumption does not increase. For future prototypes, we will need to perform theoretical verification that the power screws used to move the pseudo plane are self-locking, taking into account the thread pitch, the lead screw diameter, and the lead angle.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.35]{Assets/inventor.png}
%     \caption{A screenshot of a simulation in Autodesk Inventor showing the range of motion of Feedbackpack.}
%     \label{fig:inventor}
% \end{figure}

% \subsection{Range of Motion}
% The verification method for range of motion is by simulation using the conceptual design. \autoref{fig:inventor} shows range of motion of the conceptual design simulated in Autodesk Inventor \cite{inventor}, superimposed onto an adult male figure from The Measure of Man \cite{measureOfMan}. The figure shows simulated upper and lower bounds of the device at the far reach of the user's arm as well as a fully contracted linkage in the middle of the range of motion. This simulation demonstrates that in the plane shown, at least 70\% of the range of the human arm appears to be achievable. However, this value is estimated, not rigorously calculated in the simulation. As well, it is confounded by the consideration of the 3D range of motion of the user and by potential interference with the user's clothing and HMD. \autoref{fig:steamVRHome} attempts to find appropriate link lengths and base position for Feedbackpack, taking into account these two factors. This difficulty of weighing trade offs and attempting to design for wearability while simultaneously trying to implement motors for actuating the pseudo bounding plane is what pushed the project timeline back and prevent the fabrication of the full-scale prototype.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.4]{Assets/matlabGeometry.jpg}
%     \caption{A diagram showing the geometry and variables used for the force calculations.}
%     \label{fig:matlabGeometry}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.5]{Assets/matlab.jpg}
%     \caption{The results of a Matlab simulation calculating the internal forces and moments in the proposed mechanism.}
%     \label{fig:matlab}
% \end{figure}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.55]{Assets/crossSection.jpg}
%     \caption{A diagram of the acrylic cross section used in the stress calculations.}
%     \label{fig:crossSection}
% \end{figure}

% \subsection{Theoretical Force Tolerance}
% The verification method for theoretical force tolerance is by calculation based on the conceptual design. \autoref{fig:matlabGeometry} shows the version of the conceptual design used for the force calculations. \autoref{fig:matlab} contains Matlab \cite{matlab} plots showing the maximum internal normal forces and moments in the conceptual design linkage for values of $-\pi < \theta_2 < 0$, $\left| F_{c,Ap} \right|=700\text{N}$, and $0 < \theta_{F_c} < 2\pi$. These plots show that the points of concern are when $\theta_2$ is -$\pi$rad or 0rad. These represent robotic singularities, which Feedbackpack avoids. Therefore, the rough maximum internal forces and moments are $F_\text{max}=8000\text{N}$ and $M_{\text{max}}=300\text{Nm}$, respectively. Assuming that the maximum internal force and moment were to act at the same point on an acrylic linkage with the cross section shown in \autoref{fig:crossSection}, the following calculations find the factor of safety:\\
% Find the second moment of area.
% \begin{align*}
%     I_{xx} & = \frac{1}{12}b{h}^3 \\
%     & = \frac{1}{12}(0.016\text{m})(0.080\text{m})^3 \\
%     & = 0.1067 \times 10^{-3}\text{m}^4
% \end{align*}
% Find the maximum normal stress in the cross section.
% \begin{align*}
%     \sigma_\text{max} & = \frac{M_\text{max} y_\text{max}}{I_{xx}}+\frac{F_\text{max}}{A} \\
%     & = 6.36\text{MPa}
% \end{align*}
% The breaking stress of acrylic is $\sigma_{\text{max}_\text{acrylic}}=64.8\text{MPa}$ \cite{acrylic}. Compare the maximum stress to the breaking stress of acrylic to obtain a factor of safety.
% \begin{align*}
%     \text{Factor of Safety} & = \frac{\sigma_{\text{max}_\text{acrylic}}}{\sigma_\text{max}} \\
%     & = 10.2
% \end{align*}
% These calculations are rudimentary, and do not take into account combined loading, torsion, or other failure methods such as shear failure at joints. Additionally, the geometry and design used for these calculations does not reflect the geometry which will be used in the next prototype. However, the calculations do show that the current overall design is overdesigned. Therefore, the next prototype should focus on proving out the next set of key specifications without great concern about stress failure.

% \subsection{Specifications Not Verified with the Current Prototype}
% The narrow scope of the current prototype limited which specifications could be verified. The specifications of weight, stiffness, viscous damping, and natural frequency require a full-scale prototype for verification. The specifications of power consumption, position control overshoot, position control settling time, and other metrics like refresh rate and position control steady state error all require the implementation of the electronic actuator and controller components.
% %Guess I'm not going to go in depth about how I would verify these.

% %\section{Qualitative Feedback}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.7]{Assets/demo}
%     \caption{A set of photos showing that the primary end effector can freely engage or disengage the 2D apparent bounding plane, and slides along the 2D apparent bounding plane when engaged.}
%     \label{fig:demo}
% \end{figure}

% \section{Demo Applications} %stress ... portability
% Feedbackpack's objective is to fill the the gap in the haptics application space of passively rendering virtual planes and surfaces. The demonstrations in \autoref{fig:demo} verify that Feedbackpack fills this gap. \autoref{fig:demo} shows that the design allows the handheld end effector to freely engage with or disengage from the apparent bounding plane. The figure also shows that when the handheld end effector is engaged with the apparent bounding plane, it can freely and passively slide in two dimensions. The future Feedbackpack must demonstrate that it is able to achieve this same effect while being body grounded.
% %\subsection{Point out some features not mentioned before}
% %\subsection{Walls}
% %\subsection{Desks}
% %\subsection{Hand Stabilization for Writing and Drawing}
% %\subsection{Menu Interaction}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% How do I achieve this stiffness good tolerancing what are the issues with the tolerancing in the implementation how do I what am I talking about what are the limitations of the implementation well I suppose one of them is lake purchase parts 
% How did I do what I did well it's fairly simple I made the links the correct size that was important I used 8020 and I adjusted in hand I printed parts I spent a lot of time tolerancing I don't really know what else to say  

% The second key specification is a tolerable force of greater than 700N. The maximum force with which users are expected to be able to push forward is with the force of a bodyweight chest press. For an adult male, this is 700N. Wireality \cite{wireality}, the previous shoulder-mounted passive device, could apply 183N per finger. This totals 915N, which is on the same order of magnitude.

% The third key design specification is an effective stiffness at the end effector of greater than 20.0 N/mm. The objective of the design is to be able to render immobile planes. The stiffness of the device measured between its body grounding point and the end effector determines the perceived compliance or stiffness of the rendered surface. The metric for stiffness is obtained from combining the maximum desired force and the maximum desired deflection. The maximum desired deflection is 8mm, based on the just noticeable difference from perception research \cite{perceptionResearch}. This is further supported by the domination of vision over proprioception in VR and its applications in haptic retargeting \cite{macbeth, hapticRetargeting}. Representing Feedbackpack as a spring, the stiffness is represented by the spring constant $k$ and can be obtained from $k=F/\delta=700.0\text{N}/8.0\text{mm}=87.5\text{N/mm}$. 

% The fourth key design specification is an effective viscous damping at the end effector of less than 80kg/s. The viscous damping coefficient represent the resting impedance of the device. Feedbackpack should operate as en encountered-type device, meaning that the user should not feel any significant resistance or impedance when they are not interacting with the rendered surface. Assuming that the impedance of the device can be modelled as viscous damping, the viscous damping coefficient can be obtained from $c=F/\dot{x}$. Desiring that the user must only apply 20N to move at 250mm/s requires a viscous damping coefficient of 80kg/s.

% \subsection{Linkage Design}
% The current prototype uses rectangular cross sections for the linkages. The size of the cross section was designed for ease of rapid prototyping, rather than resulting from engineering calculations.

% The linkage design in the current prototype achieves 3DOF (degree of freedom) movement of its end effector when freely moving around and 2DOF movement of its end effector when rendering a virtual surface. The linkage design achieves this using a ball joint located inside the pin joint of the pseudo end effector. \autoref{fig:ballJoint} shows a section view of this pin joint inside a ball joint. We fabricated the three parts shown in \autoref{fig:ballJoint} at once using 3D printing. However, future prototypes will require a stronger ball joint than 3D printing filament can provide. Therefore, future designs will use a virtual scaled linkage (where a virtual link means that the link does not exist, but the same motion and effect is achieved by adding links elsewhere), as shown in \autoref{fig:conceptualDesignFuture}.

% \subsection{Hand Interface}
% The hand interface on the current prototype is a rod through a pin joint at the primary end effector. This is sufficient to prove out the conceptual design. The worn prototype will have a more natural hand interface, similar to standard handheld controllers. Based on qualitative feedback of the prior work, the hand interface should allow 6DOF movement of the hand and wrist, even though Feedbackpack will only provide 3DOF force feedback \cite{calvo}. This will increase user comfort and will increase the breadth of interactions and applications the device supports.

% \subsection{Specifications Not Achieved in the Current Prototype}
% \label{section:otherSpecs}
% The current iteration of the prototype does not address all of the specifications listed in \autoref{tab:designSpecifications}. 

% The current prototype is not body-grounded, but rather is implemented as a desktop device in order to prove out the key specifications. Feedbackpack's body grounding approach has not been finalized and will require iterative prototyping. We will first attempt to implement body grounding using backpack, chest, and waist straps, following from previous devices \cite{calvo, wireality}. This approach is shown in \autoref{fig:teaser}. If it is too difficult to control the deflection of the end effector or the straps need to be too tight than is comfortable, then we will investigate a novel active body grounding approach. This approach will use an array of pads on the upper body, in informed locations \cite{whereToWear}, connected to a stiff frame by actuators and force sensors. The sensors and actuators will use signal feedback control to apply appropriate force and moment onto the user's body. This way, Feedbackpack is not relying neither on the deformation of the user's body nor on the deformation of flexible straps to generate the reaction force. A further advantage of this active body grounding approach is that the use of feedback control may allow it to fit different users with ease. The disadvantage of this approach is that it is expensive and complex.

% The current prototype does not have VR integration. VR integration is not itself a novel feature, and so will not be implemented until the prototype is full scale. Two primary challenges associated with VR integration are position tracking and physical interference of the headset and the haptic device. The position tracking will be achieved externally using commercial infared VR trackers. This approach uses only two optical trackers, while the alternative approach would require one optical tracker and at least three position trackers at the joints of the linkage. VR headsets are bulky, and their bulk may interfere with Feedbackpack's bulk. \autoref{fig:steamVRHome} shows an attempt in a VR sketching application to design a body grounding approach to maximize range of motion and avoid collisions with the headset.

% The current prototype has no electrical components. Future prototypes will have actuators to move the pseudo bounding plane, sensors for position tracking, a microprocessor for processing, voltage regulation components, and possibly sensors and actuators for body grounding. The actuators to move the pseudo bounding plane will likely be DC motors which spin the self-locking lead screws with a high gear reduction. The simplicity of this design may come at the cost of a high noise level. A host computer will receive the optical external tracking data and will interpret the intended behaviour of the device based on the context of the virtual scene. The microprocessor must communicate with the host computer to receive actuation instructions. The refresh rate suggested by the previous work is 200Hz \cite{calvo}.




% Our objective was to design a force feedback device or paradigm which allows stiff, passive, encountered-type interactions with planes while maintaining portability by being active. We wished for our design to also be able to render irregular shapes and to have the possibility of rendering active force feedback. 

% In order to demonstrate, verify, and present our design paradigm, we created a desktop force feedback implementation of the design paradigm. This implementation can support the full range of motion of a user's arm and positions the proxy object so that the pseudoplane contact meets it directly. In this section we discuss the details and specifications of our implementation of the design paradigm.

% \subsection{Design Goals for Implementation}
% In addition to the design goals for the paradigm, we wished the implementation to have a weight on hand of less than 500 grams, to allow the user full range of motion of their arm, to be able to render an infinite horizontal plane, to be able to adjust the height of the plane at least faster than 10 centimeters per second, and to have an effective stiffness from the pseudoplane contact to the end effector of greater than 100N/mm. 


%What other requirement did you need to satisfy?
%How does the device mount to the user?
% Because the implementation is not wearable, 
%Why is that requirement important?
% This allows the user to have complete freedom of motion when they are not interacting with the plane.
%How does the user interact with the device? %What else did you do to make it easier to use (vest)

%How do you ensure no 'line of sight'/'occlusion'/'clipping' problems? 
%How do your choices relate to comfort?
%How do your choices relate to body grounding the forces
%Did you consult anything about wear location?






%What did you make?
% We produced a set of applications corresponding to a set of implementations of the design paradigm. The applications, shown in Figure \ref{fig:DemoApplications}, are a table (a horizontal plane), a table in a simulation of a wearable implementation, two walls (vertical planes) meeting at a corner, a rough surface, an irregular surface profile, a horizontal spring, constant weight, and a pencil and paper application.
% The horizontal plane demonstrates that the user can freely move their hand around the space when they are not engaging the plane, that the interaction with the plane is stiff, that the interaction with the plane is encountered-type and allows sliding across the plane, and that the scaling mechanism handles tapping interactions well.
% In the simulation of a wearable implementation, wizard of oz operators change the height of the device as the user changes their torso height. This application demonstrates that the device can compensate for the user movement and can adjust the local height of the plane so that the perceived table stays at a consistent height in the simulation. 
% The vertical plane shows that all of the the features regarding horizontal planes can also be demonstrated for vertical planes. 
% The pencil and paper application demonstrates the potential of enabling VR users to stabilize their hand in midair, allowing them to perform fine motor tasks which are currently challenging in VR.
%Who is experiencing the demo?
% Each of the study participants had the opportunity to experience the demo following their participation in the study. 
%What does your device do in the demo?
% For each use case in the demo, an implementation of our device passively renders the plane, surface, or force being demonstrated.
%What is the experience of the user?
% For each application and implementation, the user has as much time as they wish for exploration. Once the user wishes to move on to the next application, they doff the device and HMD and we set up the next implementation. 



%What supplementary work did you have to do to realize the demo?
% In order to realize the demo, we had to create a vertical plane attachment for the pseudoplane, a rough film attachment for the pseudoplane, an irregular surface attachment for the pseudoplane, a spring attachment for the pseudoplane joint, a constant force spring attachment for the pseudoplane joint, and a gimbal and controller holder for the end effector.
%What are the details of that effect?
% Because the pseudoplane joint is mechanically linked to and is related by scaling to the end effector, any force or positional constraint at the pseudoplane joint is multiplied and felt by the end effector.
%What are the details of that implementation
% The vertical planes were constructed of 8020. The rough film was carpet. The irregular surface was 3D printed. The constant force spring was a custom coiled piece of sheet metal. The gimbal and controller holder were 3D printed.
%How long does it take for the device to change its shape?
% Because of the specific implementation, the device can only adjust the height of the rendered plane at a speed of \{10cm/s\}. Therefore, it can only compensate for user movement slower than or equal to that speed. Other designs and implementations of the paradigm will be able to maintain the passivity of the interaction while adjusting at a greater rate.
%What is the consequence of the amount of time it takes for the device to change its shape? %What happens when the user presses very hard? 
% In each of the demonstrations showing a passive interaction, when the user presses very hard, the change in displacement is due only to the flexibility of the members used in the implementation.
%What value does the interactivity have? %Can the user change the state of the world? Is this different than if there was no force feedback?



% I we had not used a lead screw, then the actuation system would not have been mechanically self locking and the motor would have needed to activate to keep the pseudoplane stationary whenever the user interacted with it. If we had used a stepper motor then the motor would not have been able to overcome the force required to turn the lead screw. If we had used a servo motor, then the motor would not have had enough turns to travel the pseudoplane a sufficient distance. 
%What did you initially do?
%What problems initially arose?



%How did you control the system? %What motor drivers did you use? %What controller did you use?

%How did this relate to your design goals? 
%What advantages does your final design offer?
%What are some numbers or math bits?
% The motors were  DC motors . The lead screws were from a kit and had a certain lead angle and pitch. We used guide rails from the same kit to guide the pseudoplane.
%What problem would occur if you did not have this thing? 


